Noisy Submodular Maximization via Adaptive Sampling with Applications to Crowdsourced Image Collection Summarization

We address the problem of maximizing an unknown submodular function that can only be accessed via noisy evaluations. Our work is motivated by the task of summarizing content, e.g., image collections, by leveraging users' feedback in form of clicks or ratings. For summarization tasks with the goal of maximizing coverage and diversity, submodular set functions are a natural choice. When the underlying submodular function is unknown, users' feedback can provide noisy evaluations of the function that we seek to maximize. We provide a generic algorithm -- \submM{} -- for maximizing an unknown submodular function under cardinality constraints. This algorithm makes use of a novel exploration module -- \blbox{} -- that proposes good elements based on adaptively sampling noisy function evaluations. \blbox{} is able to accommodate different kinds of observation models such as value queries and pairwise comparisons. We provide PAC-style guarantees on the quality and sampling cost of the solution obtained by \submM{}. We demonstrate the effectiveness of our approach in an interactive, crowdsourced image collection summarization application.

==> experiments_featureSel.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Additional Experiments --- Feature Selection}
\label{app.feat_sel}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[t!]
\centering
   \subfigure[Information gain]{
     \includegraphics[width=0.31\textwidth]{fig/results_featureSel_ig.pdf}
     \label{fig.resuts1.syn2}
   }
   \subfigure[Species]{
     \includegraphics[width=0.31\textwidth]{fig/fig_featureSel_Task.pdf}
     \label{fig.resuts1.syn1}
   }   
   \subfigure[Classification accuracy]{
     \includegraphics[width=0.31\textwidth]{fig/results_featureSel_accuracy.pdf}
    \label{fig.resuts1.syn3}
   }
\caption{Results from synthetic simulations for feature selection.} 
\label{fig.resuts1_fs}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this section we provide additional experiments for feature selection. We first describe the task in more detail and then present our experimental results.

\subsection{Objective} 
For this task we used the \emph{Caltech-UCSD Birds-200-2011} image dataset with photos of 200 bird species~\cite{WahCUB_200_2011}.
Each image in this dataset was annotated with 312 binary attributes, e.g.\ \emph{has\_forehead\_color:red}, through workers on MTurk. Features can take values in \{+1, -1 \} indicating the presence or absence of an attribute.
We considered a binary classification task of endandegred vs. non-endagnered woodpeckers, cf.\ Figure~\ref{fig.resuts1_fs}(b).  A similar setting was considered in~\cite{singla14crowdteaching} in the context of crowdsourcing experimentation.
% $[2013-cvpr_DengKrauseFei-Fei_fine-grained-crowdsourcing]$ used the same dataset to elicit features by designing a visual game.
We reduced the 312 features to a total of 10 features as follows: We took the 3 most informative features according to a binary naive-Bayes model for classification. Additionally, we selected 3 features that were redundant to the already selected ones, e.g.\ \emph{has\_forehead\_color:red} and \emph{has\_forehead\_color:black}. We randomly sampled the remaining 4 other features. 

From these features we built a naive-Bayes classifier and used the corresponding information gain as the submodular function for our experiments.

\subsection{Results via Simulations}

Our results for the synthetic experiments for feature selection are shown in Figure~\ref{fig.resuts1_fs}. 
In our first experiment, we compare the quality of solutions obtained by algorithm $\textsc{SubmSelX}^P$ to solutions of the greedy algorithm. The utility of the sets selected during execution of the algorithm are shown in Figure~\ref{fig.resuts1_fs}(a). The results are qualitatively the same as for the image collection summarization task, as reported earlier. Here, we also computed the classification accuracy as  metric of real interest for real, cf.\ Figure~\ref{fig.resuts1_fs}(c).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


